Signal shapes in multiwire proportional chamber-based TPCs

A large-volume Time Projection Chamber (TPC) is the main tracking and particle identification (PID) detector of the ALICE experiment at the CERN LHC. PID in the TPC is performed via specific energy-loss measurements (dE/dx), which are derived from the average pulse-height distribution of ionization generated by charged-particle tracks traversing the TPC volume. During Runs 1 and 2, until 2018, the gas amplification stage was based on multiwire proportional chambers (MWPC). Signals from the MWPC show characteristic long negative tails after an initial positive peak due to the long ion drift times in the MWPC amplification region. This so-called ion tail can lead to a significant amplitude loss in subsequently measured signals, especially in the high-multiplicity environment of high-energy Pb-Pb collisions, which results in a degradation of the dE/dx resolution. A detailed study of the signal shapes measured with the ALICE TPC with the Ne-CO2 (90-10) and Ar-CO2 (90-10) gas mixtures is presented, and the results are compared with three-dimensional Garfield simulations. The impact of the ion tail on the PID performance is studied employing the ALICE simulation framework and the feasibility of an offline correction procedure to account for the ion tail is demonstrated.

==> Authors_JINST_FINAL.tex <==
\affiliation[1]{Bose Institute, Department of Physics  and Centre for Astroparticle Physics and Space Science (CAPSS), Kolkata, India}
\affiliation[2]{Comenius University Bratislava, Faculty of Mathematics, Physics and Informatics, Bratislava, Slovakia}
\affiliation[3]{Department of Physics, University of Oslo, Oslo, Norway}
\affiliation[4]{Department of Physics and Technology, University of Bergen, Bergen, Norway}
\affiliation[5]{European Organization for Nuclear Research (CERN), Geneva, Switzerland}
\affiliation[6]{Faculty of Engineering and Science, Western Norway University of Applied Sciences, Bergen, Norway}
\affiliation[7]{Helmholtz-Institut f\"{u}r Strahlen- und Kernphysik, Rheinische Friedrich-Wilhelms-Universit\"{a}t Bonn, Bonn, Germany}
\affiliation[8]{Helsinki Institute of Physics (HIP), Helsinki, Finland}
\affiliation[9]{High Energy Physics Group, Universidad Aut\'{o}noma de Puebla, Puebla, Mexico}
\affiliation[10]{Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest, Romania}
\affiliation[11]{Indian Institute of Technology Bombay (IIT), Mumbai, India}
\affiliation[12]{Institut f\"{u}r Kernphysik, Johann Wolfgang Goethe-Universit\"{a}t Frankfurt, Frankfurt, Germany}
\affiliation[13]{Instituto de Ciencias Nucleares, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Mexico City, Mexico}
\affiliation[14]{Lund University Department of Physics, Division of Particle Physics, Lund, Sweden}
\affiliation[15]{Nagasaki Institute of Applied Science, Nagasaki, Japan}
\affiliation[16]{Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark}
\affiliation[17]{Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA}
\affiliation[18]{Physics department, Faculty of science, University of Zagreb, Zagreb, Croatia}
\affiliation[19]{Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}
\affiliation[20]{Physik Department, Technische Universit\"{a}t M\"{u}nchen, Munich, Germany}
\affiliation[21]{Research Division and ExtreMe Matter Institute EMMI, GSI Helmholtzzentrum f\"ur Schwerionenforschung GmbH, Darmstadt, Germany}
\affiliation[22]{The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland}
\affiliation[23]{The University of Texas at Austin, Austin, Texas, USA}
\affiliation[24]{Universidade de S\~{a}o Paulo (USP), S\~{a}o Paulo, Brazil}
\affiliation[25]{University of Houston, Houston, Texas, USA}
\affiliation[26]{University of Tennessee, Knoxville, Tennessee, USA}
\affiliation[27]{University of Tokyo, Tokyo, Japan}
\affiliation[28]{Variable Energy Cyclotron Centre, Kolkata, India}
\affiliation[29]{Wigner Research Centre for Physics, Budapest, Hungary}
\affiliation[30]{Yale University, New Haven, Connecticut, USA}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\author[4]{J.~Alme,}
\author[12]{T.~Alt,}
\author[10]{C.~Andrei,}
\author[19]{V.~Anguelov,}
\author[12]{H.~Appelsh\"{a}user,}
\author[30,*]{M.~Arslandok, \note[*]{Corresponding authors}}\emailAdd{mesut.arslandok@cern.ch}
\author[29]{G.G.~Barnaf\"{o}ldi,}
\author[12]{E.~Bartsch,}
\author[19,21]{P.~Becht,}
\author[25]{R.~Bellwied,}
\author[19]{A.~Berdnikova,}
\author[12]{N.~Bialas,} 
\author[12]{P.~Bialas,}  
\author[1]{S.~Biswas,}
\author[19,21]{B.~Blidaru,}
\author[29]{L.~Boldizs\'{a}r,}
\author[12]{L.~Bratrud,}
\author[21]{P.~Braun-Munzinger,}
\author[24]{M.~Bregant,}
\author[17]{C.L.~Britton,} 
\author[19]{S.~Brucker,}
\author[8]{E.J.~Br\"{u}cken,} 
\author[12]{H.~B\"{u}sching,}
\author[30]{H.~Caines,}
\author[9]{R.~Soto Camacho,} 
\author[26]{A.J.~Castro,} 
\author[19]{P.~Chatzidaki,}
\author[14]{P.~Christiansen,}
\author[17]{L.G.~Clonts,} 
\author[17,\dagger]{T.M.~Cormier, \note[$\dagger$]{Deceased}}
\author[11]{P.~Dhankher,}
\author[12]{S.~Dittrich,} 
\author[30]{R.~Ehlers,}
\author[17]{M.N.~Ericson,} 
\author[17]{N.B.~Ezell,} 
\author[20]{L.~Fabbietti,}
\author[25]{F.~Flor,}
\author[16]{J.J.~Gaardh{\o}je,}
\author[24]{M.G.~Munhoz,}
\author[21]{C.~Garabatos,}
\author[21]{P.~Gasik,}
\author[12]{T.~Geiger,} 
\author[29]{\'{A}.~Gera,} 
\author[19]{P.~Gl\"{a}ssel,}
\author[15]{D.J.Q.~Goh,}
\author[12]{A.~Grein,}
\author[12]{T.~Gundem,}
\author[27]{T.~Gunji,}
\author[21]{M.~Habib,}
\author[15]{H.~Hamagaki,}
\author[29]{G.~Hamar,} 
\author[16]{J.C.~Hansen,}
\author[30]{J.W.~Harris,}
\author[7]{P.~Hauer,}
\author[27]{S.~Hayashi,}
\author[21]{J.~Hehner,} 
\author[8]{J.K.~Heino,}
\author[12]{E.~Hellb\"{a}r,}
\author[6]{H.~Helstrup,}
\author[12]{M.~Hemmer,}
\author[10]{A.~Herghelegiu,} 
\author[24]{R.A.~Hernandez,} 
\author[24]{H.D.~Hernandez Herrera,} 
\author[8]{T.E.~Hilden,}
\author[26]{C.~Hughes,}
\author[19]{S.~Hummel,}
\author[21,*]{M.~Ivanov,} \emailAdd{marian.ivanov@cern.ch}
\author[12]{J.~J\"{a}ger,}
\author[12]{J.~Jung,}
\author[12]{M.~Jung,}
\author[8]{E.~Kangasaho,}
\author[7]{B.~Ketzer,}
\author[12]{S.~Kirsch,}
\author[12]{M.~Kleiner,}
\author[20]{T.~Klemenz,}
\author[25]{A.G.~Knospe,}
\author[22]{M.~Kowalski,}
\author[21]{L.~Kreis,}
\author[12]{M.~Kr\"{u}ger,}
\author[19]{N.~Kupfer,} 
\author[20]{R.~Lang,}
\author[20]{L.~Lautner,}
\author[20]{M.~Lesch,}
\author[5]{Y.~Lesenechal,} 
\author[12]{F.~Liebske,}
\author[21]{C.~Lippmann,}
\author[30,\dagger]{R.D.~Majka,}
\author[23]{C.~Markert,}
\author[24]{T.A.~Martins,} 
\author[21]{S.~Masciocchi,}
\author[14]{O.~Matonoha,}
\author[22]{A.~Matyja,}
\author[2]{M.~Meres,}
\author[20]{D.L.~Mihaylov,}
\author[21]{D.~Mi\'{s}kowiec,}
\author[19]{T.~Mittelstaedt,}
\author[20]{C.~Mordasini,}
\author[21]{T.~Morhardt,} 
\author[19]{S.~Muley,} 
\author[30]{J.~Mulligan,}
\author[12]{R.H.~Munzer,}
\author[27]{H.~Murakami,}
\author[7]{K.~M\"{u}nning,} 
\author[14]{A.~Nassirpour,}
\author[26]{C.~Nattrass,}
\author[16]{B.S.~Nielsen,}
\author[24]{W.A.V.~Noije,}  
\author[15]{M.~Ogino,}
\author[26]{A.C.~Oliveira Da Silva,}
\author[14]{A.~Oskarsson,} 
\author[15]{K.~Oyama,}
\author[14]{A.~\"Onnerstad,}
\author[14]{L.~\"Osterman,} 
\author[19]{Y.~Pachmayer,}
\author[13]{G.~Pai\'{c},}
\author[28]{R.N.~Patra,}
\author[12]{V.~Peskov,} 
\author[10]{M.~Petris,} 
\author[10]{M.~Petrovici,}
\author[2]{M.~Pikna,}
\author[18]{M.~Planinic,}
\author[10]{L.~Prodan,} 
\author[10]{A.~Radu,} 
\author[17]{J.~Rasson,} 
\author[17]{K.F.~Read,}
\author[4]{A.~Rehman,}
\author[12]{R.~Renfordt,} 
\author[3]{K.~R{\o}ed,}
\author[4]{D.~R\"ohrich,}
\author[19]{E.~Rubio,} 
\author[17]{A.~Rusu,}
\author[24]{B.C.S.~Sanches,} 
\author[23]{J.~Schambach,}
\author[12]{S.~Scheid,}
\author[21]{C.~Schmidt,}
\author[26]{A.~Schmier,}
\author[21]{K.~Schweda,}
\author[27]{D.~Sekihata,}
\author[19]{S.~Siebig,} 
\author[24]{R.W.D.~Silva,} 
\author[14]{D.~Silvermyr,}
\author[2]{B.~Sitar,}
\author[30]{N.~Smirnov,}
\author[19]{H.K.~Soltveit,} 
\author[21]{C.~Sonnabend,} 
\author[26]{S.P.~Sorensen,} 
\author[19]{J.~Stachel,}
\author[20]{L.~\v{S}erk\v{s}nyt\.{e},}
\author[4]{G.~Tambave,}
\author[4]{K.~Ullaland,}
\author[20]{B.~Ulukutlu,}
\author[29]{D.~Varga,}
\author[14]{O.~Vazquez Rueda,}
\author[4]{A.~Velure,} 
\author[9]{S.~Vergara Lim\'on,}
\author[19]{O.~Vorbach,} 
\author[21]{B.~Voss,}
\author[12]{C.~Weidlich,} 
\author[12]{J.~Wiechula,}
\author[19]{B.~Windelband,}
\author[20]{S.~Winkler} 
\author[19]{F.~Zanone} 
%\corref{cor1,},} \ead{andreas.mathis@ph.tum.de,}
%\cortext[dec]{deceased,}



